Exploiting Asymmetry for Synthetic Training Data Generation: SynthIE and the Case of Information Extraction

Large language models (LLMs) have great potential for synthetic data generation. This work shows that useful data can be synthetically generated even for tasks that cannot be solved directly by LLMs: for problems with structured outputs, it is possible to prompt an LLM to perform the task in the reverse direction, by generating plausible input text for a target output structure. Leveraging this asymmetry in task difficulty makes it possible to produce large-scale, high-quality data for complex tasks. We demonstrate the effectiveness of this approach on closed information extraction, where collecting ground-truth data is challenging, and no satisfactory dataset exists to date. We synthetically generate a dataset of 1.8M data points, establish its superior quality compared to existing datasets in a human evaluation, and use it to finetune small models (220M and 770M parameters), termed SynthIE, that outperform the prior state of the art (with equal model size) by a substantial margin of 57 absolute points in micro-F1 and 79 points in macro-F1. Code, data, and models are available at https://github.com/epfl-dlab/SynthIE.

==> bucket-plot_num-target-triplets.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=0.8\columnwidth]{plots/bucket-plot_num-target-triplets/bucket-plot-num-target-triplets_models-genie-base--synthie-base_datasets-rebel--syntext_vertical_f1.pdf}
    \vspace{-1em}
    \caption{\textbf{F1-vertical.TODO}}
    \label{fig:bucket_plot}
\end{figure*}






==> bucket-plot_rel-occ_f1.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{plots/bucket-plot_rel-occ/bucket-plot_models-genie-base--synthie-base_datasets-rebel--syntext_f1.pdf}
    \vspace{-1em}
    \caption{\textbf{Impact of the number of relation occurrences.} Relations are bucketed based on their number of occurrences; bucket $2^i$ contains relations occurring between $2^{i}$ and $2^{i+1}$ times. The histogram shows the number of relations per bucket. The line plots depict the F1 scores for GenIE and SynthIE per bucket, with confidence intervals constructed by bootstrap resampling. TODO: Add takeaway for the plot.}
    \label{fig:bucket_plot}
\end{figure*}




==> bucket-plot_rel-occ_recall.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{plots/bucket-plot_rel-occ/bucket-plot_models-genie-base--synthie-base_datasets-rebel--syntext_recall.pdf}
    \vspace{-1em}
    \caption{\textbf{Impact of the number of relation occurrences.} Relations are bucketed based on their number of occurrences; bucket $2^i$ contains relations occurring between $2^{i}$ and $2^{i+1}$ times. The histogram shows the number of relations per bucket. The line plots depict the Recall scores for GenIE and SynthIE per bucket, with confidence intervals constructed by bootstrap resampling. TODO: Add takeaway for the plot.}
    \label{fig:bucket_plot}
\end{figure*}



==> human_eval_plots_task1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{plots/human_eval_plots/human_eval_task1_plot.pdf}
    \vspace{-1em}
    \caption{\textbf{SDG quality analysis.} Bar plot shows results for original data (REBEL), \sdgCodeDataset{} data, and \sdgTextDataset{} data with 95\% confidence intervals. \emph{Left:} Results of human evaluation assessing precision for synthetic data generation. \emph{Right:} Results of manual analysis assessing recall for synthetic data generation. }
    \label{fig:human_eval_task1}
\end{figure}

==> human_eval_plots_task2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{plots/human_eval_plots/human_eval_task2_plot.pdf}
    \vspace{-1em}
    \caption{\textbf{SynthIE human evaluation.} \emph{Left:} Precision. \emph{Right:} Relative recall.}
    \label{fig:human_eval_task2}
\end{figure}

==> human_eval_task2_table.tex <==
\begin{table}[t]
\centering
\resizebox{0.43\textwidth}{!}{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lccc@{}}
\toprule
& \multicolumn{3}{c}{REBEL$^{++}$} \\
& Precision & Recall & F1 \\

\midrule
\midrule

\multicolumn{3}{l}{\emph{\textbf{Micro}}} \\ 
\hspace{4mm} REBEL{\footnotesize~{Gold}} & 89.93 {\scriptsize± 1.98} & 60.46 {\scriptsize± 2.67} & 72.72 {\scriptsize± 2.12} \\
\midrule
\hspace{4mm} GenIE{\footnotesize~{T5-base}} & 72.91 {\scriptsize± 3.56} & 51.24 {\scriptsize± 3.02} & 60.70 {\scriptsize± 2.77} \\
\midrule
\hspace{4mm} SynthIE{\footnotesize~{T5-base}} & 51.65 {\scriptsize± 4.39} & 43.73 {\scriptsize± 3.02} & 47.79 {\scriptsize± 3.16} \\
\hspace{4mm} SynthIE{\footnotesize~{T5-base-SC}} & 58.53 {\scriptsize± 4.18} & 30.72 {\scriptsize± 1.97} & 40.58 {\scriptsize± 2.39} \\
\hspace{4mm} SynthIE{\footnotesize~{T5-large}} & 66.47 {\scriptsize± 4.34} & 54.91 {\scriptsize± 3.01} & 60.87 {\scriptsize± 2.83} \\

\midrule
\midrule

\emph{\textbf{Macro}} \\ 
\hspace{4mm} REBEL{\footnotesize~{Gold}} & 49.76 {\scriptsize± 5.05} & 41.11 {\scriptsize± 4.48} & 43.05 {\scriptsize± 4.53} \\
\midrule
\hspace{4mm} GenIE{\footnotesize~{T5-base}} & 37.08 {\scriptsize± 4.56} & 30.74 {\scriptsize± 3.97} & 31.93 {\scriptsize± 3.92} \\
\midrule
\hspace{4mm} SynthIE{\footnotesize~{T5-base}} & 33.98 {\scriptsize± 4.17} & 34.41 {\scriptsize± 4.01} & 32.26 {\scriptsize± 3.82} \\
\hspace{4mm} SynthIE{\footnotesize~{T5-base-SC}} & 19.21 {\scriptsize± 2.78} & 12.57 {\scriptsize± 2.39} & 14.23 {\scriptsize± 2.39} \\
\hspace{4mm} SynthIE{\footnotesize~{T5-large}} & 50.35 {\scriptsize± 4.57} & 50.66 {\scriptsize± 4.47} & 48.25 {\scriptsize± 4.30} \\
\bottomrule                         
\end{tabular}
}
\caption{\textbf{Performance on the human\hyp annotated subset of REBEL.} REBEL{\footnotesize~{Gold}} scores critically low. In terms of macro, REBEL's \textit{ground truth} is of comparable quality with SynthIE{\footnotesize~{T5-large}}'s \textit{predictions}.}
\label{tab:human_eval_2}
\end{table}

==> old_05_experiments_and_results.tex <==
\section{Experiments and Results}


\subsection{Performance Evaluation}


RQ2.1: (Coarse Analysis) Does the proposed approach improve overall performance (Micro/Macro Precision, Recall, F1)?

RQ2.2: (Fine-grained Analysis) Analysis of performance as a function of the relation occurrence count?

Entities: GenIE (max entities in the training set + evaluation set)
Relations: GenIE (max relations in the training set ?)

Baseline: FlanT5 (300 mil) trained only data from the training set

New model: Same model trained on both(?) data from the training set and synthetic data

Evaluation: Automatic

\subsection{Human evaluation}
\label{sec:human_eval_synthie}

\marija{why we do human evaluation}

\xhdr{Task setup}
To evaluate the performance of SynthIE in comparison to the ground truth (REBEL), we take 51 randomly sampled sentence from REBEL samples and use SynthIE to generate the facts present in them. This results in two sentence-facts set pairs, one originating from REBEL, and one from our model. We evaluate these pairs by two metrics, \emph{precision} (see \Secref{sec:sgd_quality}) and \emph{relative recall}. To evaluate precision, we recruit workers from MTurk using the same task setting and crowdsourcing criteria as in~\Secref{sec:exhaustiveness}. Relative recall is then calculated as follows: for a sampled sentence, estimated ground truth facts set is obtained by taking a union of the outcome facts set from the task performed on MTurk for both REBEL and SynthIE sample. Relative recall for each sample is calculated by dividing number of triplets workers marked in the MTurk task with the number of triplets in the estimated ground truth facts set.

\xhdr{Results}
In~\Figref{fig:human_eval_task2} we present precision (left) and relative recall (right) for REBEL and SynthIE. SynthIE and REBEL are indistinguishable when it comes to relative recall, with scores 58.92\% [48.59\%, 68.52\%] and 56.43\% [47.31\%, 64.83\%] respectively. SynthIE has a precision score 56.62\% [46.83\%, 66.17\%], while REBEL has 72.61\% [61.08\%, 81.66\%]. \marija{add the discussion for precision, possible examples in appendix to show why this happens.}









